STUNT: Few-shot Tabular Learning with Self-generated Tasks from Unlabeled Tables

Learning with few labeled tabular samples is often an essential requirement for industrial machine learning applications as varieties of tabular data suffer from high annotation costs or have difficulties in collecting new samples for novel tasks. Despite the utter importance, such a problem is quite under-explored in the field of tabular learning, and existing few-shot learning schemes from other domains are not straightforward to apply, mainly due to the heterogeneous characteristics of tabular data. In this paper, we propose a simple yet effective framework for few-shot semi-supervised tabular learning, coined Self-generated Tasks from UNlabeled Tables (STUNT). Our key idea is to self-generate diverse few-shot tasks by treating randomly chosen columns as a target label. We then employ a meta-learning scheme to learn generalizable knowledge with the constructed tasks. Moreover, we introduce an unsupervised validation scheme for hyperparameter search (and early stopping) by generating a pseudo-validation set using STUNT from unlabeled data. Our experimental results demonstrate that our simple framework brings significant performance gain under various tabular few-shot learning benchmarks, compared to prior semi- and self-supervised baselines. Code is available at https://github.com/jaehyun513/STUNT.

==> tables/fewshotv2.tex <==
\begin{table}[t]
\caption{
Few-shot test accuracy (\%) on 8 datasets from the OpenML-CC18 benchmark~\citep{bishcl2018openml}.
We report the mean test accuracy over 100 different seeds. Checkmark 
\checkmark~indicates the use of 100 additional labeled samples for validation (Val.), including hyperparameter searching and early stopping.
The bold denotes the highest mean score.
}

\centering
\label{tab:fewshot}
\resizebox{\textwidth}{!}{
\begin{tabular}{llc|ccccccccc}
\toprule
Type                           & \multicolumn{1}{l|}{Method}& Val.          & income          & cmc            & karhunen       & optdigit       & diabetes       & semeion        & pixel          & \multicolumn{1}{c|}{dna}            & Avg.            \\ \midrule
\multicolumn{12}{c}{\cellcolor[HTML]{EFEFEF}\# shot $=$ 1}                                                                                                                                                                                            \\ \midrule
                               & \multicolumn{1}{l|}{CatBoost}&\checkmark        & 57.00          & 34.60          & 55.67          & 61.32          & 60.02          & 43.21          & 59.16          & \multicolumn{1}{c|}{41.35}          & 52.06          \\
                               & \multicolumn{1}{l|}{MLP}& \checkmark            & 60.52          & 35.06          & 48.67          & 61.02          & 57.25          & 40.88          & 55.62          & \multicolumn{1}{c|}{44.39}          & 50.43          \\
                               & \multicolumn{1}{l|}{kNN}& -            & 61.22          & 34.99          & 54.42          & 65.58          & 58.56          & 44.35          & 61.48          & \multicolumn{1}{c|}{42.67}          & 52.82          \\
\multirow{-4}{*}{Sup.}         & \multicolumn{1}{l|}{LR}& \checkmark             & 59.64          & 35.08          & 55.05          & 65.19          & 57.61          & 42.90          & 59.71          & \multicolumn{1}{c|}{44.28}          & 52.43          \\ \midrule
                               & \multicolumn{1}{l|}{Mean Teacher}& \checkmark   & 60.63          & 35.58          & 54.57          & 66.10          & 58.05          & 43.56          & 61.02          & \multicolumn{1}{c|}{46.58}          & 53.26          \\
                               & \multicolumn{1}{l|}{ICT}&\checkmark             & 61.83          & 36.53          & 58.37          &  69.12     & 58.08          & 43.48          & 60.88          & \multicolumn{1}{c|}{46.55}               & 54.36          \\
                               & \multicolumn{1}{l|}{Pseudo Label}& \checkmark   & 60.52          & 34.97          & 49.44          & 61.50          & 57.03          & 41.42          & 56.12          & \multicolumn{1}{c|}{44.26}          & 50.66          \\
                               & \multicolumn{1}{l|}{MPL}& \checkmark            & 60.85          & 35.13          & 47.66          & 61.52          & 57.39          & 41.82          & 56.01          & \multicolumn{1}{c|}{44.22}          & 50.58          \\
\multirow{-5}{*}{Semi-sup.}    & \multicolumn{1}{l|}{VIME-Semi}& \checkmark      & 56.40          & 32.97          & 57.40          & 66.85          & 58.16          &   40.43    &   52.86   & \multicolumn{1}{c|}{39.18}               &   50.53      \\ \midrule
                               & \multicolumn{1}{l|}{SubTab~+~Fine-tune}&\checkmark & 59.74          & 35.65          & 41.11          & 49.88          & 59.35          & 30.49          & 42.23           & \multicolumn{1}{c|}{40.86}          & 44.91        \\
                               & \multicolumn{1}{l|}{SubTab~+~kNN}& -     & 61.58          & 35.87          & 48.74          & 66.05          & 59.22          & 39.99          & 61.30          & \multicolumn{1}{c|}{44.16}          & 52.36          \\
                               & \multicolumn{1}{l|}{SubTab~+~LR}& \checkmark      & 61.88          & 35.68          & 50.32          & 67.05          & 58.06          & 40.27          & 60.40          & \multicolumn{1}{c|}{45.68}          & 52.42          \\
                               & \multicolumn{1}{l|}{VIME~+~Fine-tune}&\checkmark   & 60.50          & 34.98          & 47.50          & 61.31          & 57.23          & 41.09          & 53.79          & \multicolumn{1}{c|}{44.30}          & 50.09          \\
                               & \multicolumn{1}{l|}{VIME~+~kNN}& -       & 62.16          & 35.55          & 58.56          & 69.31          & 58.35          & 46.99          & 64.62          & \multicolumn{1}{c|}{50.29}          & 55.78          \\
\multirow{-6}{*}{Self-sup.}    & \multicolumn{1}{l|}{VIME~+~LR}& \checkmark        & 61.99          & 35.30          & 59.62          & 70.52          & 56.95          & 47.20          & 64.17          & \multicolumn{1}{c|}{51.36}          & 55.89          \\ \midrule
                               & \multicolumn{1}{l|}{CACTUs}& -         & \textbf{64.02} & 36.10          & 65.59          & 71.98          & 58.92          & 48.96          & 67.61          & \multicolumn{1}{c|}{65.93}          & 59.89          \\
\multirow{-2}{*}{Unsup.-Meta.} & \multicolumn{1}{l|}{\textbf{STUNT (Ours)}}& -           & 63.52          & \textbf{37.10} & \textbf{71.20} & \textbf{76.94} & \textbf{61.08} & \textbf{55.91} & \textbf{79.05} & \multicolumn{1}{c|}{\textbf{66.20}} & \textbf{63.88} \\ \midrule
\multicolumn{12}{c}{\cellcolor[HTML]{EFEFEF}\# shot $=$ 5}                                                                                                                                                                                            \\ \midrule
                               & \multicolumn{1}{l|}{CatBoost}& \checkmark       & 64.51          & 39.75          & 82.38          & 84.05          & 65.75          & 68.69          & 84.49          & \multicolumn{1}{c|}{63.46}          & 69.14          \\
                               & \multicolumn{1}{l|}{MLP}& \checkmark           & 66.25          & 37.40          & 77.56          & 83.30          & 64.32          & 66.25          & 81.97          & \multicolumn{1}{c|}{59.73}          & 67.10          \\
                               & \multicolumn{1}{l|}{kNN}& -            & 70.49          & 38.56          & 79.98          & 84.89          & 67.32          & 68.33          & 84.02          & \multicolumn{1}{c|}{61.45}          & 69.38          \\
\multirow{-4}{*}{Sup.}         & \multicolumn{1}{l|}{LR}& \checkmark             & 66.53          & 37.15          & 81.02          & 86.22          & 64.19          & 67.87          & 85.02          & \multicolumn{1}{c|}{58.88}          & 68.36          \\ \midrule
                               & \multicolumn{1}{l|}{Mean Teacher}& \checkmark   & 67.05          & 37.73          & 81.08          & 86.66          & 65.45          & 69.67          & 85.24          & \multicolumn{1}{c|}{61.47}          & 69.29          \\
                               & \multicolumn{1}{l|}{ICT}& \checkmark            & 70.13          & 38.09          & 84.58          & 87.01         & 65.47          & 70.26          & 86.12          & \multicolumn{1}{c|}{63.37}          & 70.63         \\
                               & \multicolumn{1}{l|}{Pseudo Label}&\checkmark    & 66.26          & 37.49          & 78.60          & 83.71          & 64.46          & 67.49          & 82.94          & \multicolumn{1}{c|}{60.06}          & 67.63          \\
                               & \multicolumn{1}{l|}{MPL}& \checkmark            & 67.61          & 37.47          & 77.85          & 83.70          & 64.51          & 67.08          & 82.39          & \multicolumn{1}{c|}{59.65}          & 67.53          \\
\multirow{-5}{*}{Semi-sup.}    & \multicolumn{1}{l|}{VIME-Semi}& \checkmark      & 65.13          & 37.32          & 80.53          & 87.13         &   65.39   &     64.80    &      82.83  & \multicolumn{1}{c|}{52.08}               &  66.90     \\ \midrule
                               & \multicolumn{1}{l|}{SubTab~+~Fine-tune}& \checkmark & 66.01          & 37.60          & 67.80          & 75.40          & 66.69          & 56.46          & 75.34          & \multicolumn{1}{c|}{55.62}          & 62.62          \\
                               & \multicolumn{1}{l|}{SubTab~+~kNN}& -      & 71.91          & 39.51          & 69.56          & 83.60          & 68.79          & 59.87          & 80.13          & \multicolumn{1}{c|}{61.57}          & 66.87          \\
                               & \multicolumn{1}{l|}{SubTab~+~LR}& \checkmark      & 70.12          & 37.67          & 73.25          & 86.07          & 64.92          & 61.34          & 82.14          & \multicolumn{1}{c|}{58.90}          & 66.80          \\
                               & \multicolumn{1}{l|}{VIME~+~Fine-tune}& \checkmark  & 65.97          & 37.25          & 77.82          & 83.13          & 64.40          & 63.63          & 81.01          & \multicolumn{1}{c|}{59.58}          & 66.60          \\
                               & \multicolumn{1}{l|}{VIME~+~kNN}& -       & 72.16          & 39.28          & 79.15          & 83.86          & 66.94          & 68.45          & 84.07          & \multicolumn{1}{c|}{71.09}          & 70.63          \\
\multirow{-6}{*}{Self-sup.}    & \multicolumn{1}{l|}{VIME~+~LR}& \checkmark        & 67.80          & 37.51          & 82.87          & 87.42          & 64.29          & 71.53          & 86.79          & \multicolumn{1}{c|}{69.62}          & 70.98          \\ \midrule
                               & \multicolumn{1}{l|}{CACTUs}& -         & 72.03          & 38.81          & 82.20          & 85.92          & 66.79          & 65.00          & 85.25          & \multicolumn{1}{c|}{\textbf{81.52}} & 72.19          \\
\multirow{-2}{*}{Unsup.-Meta.} & \multicolumn{1}{l|}{\textbf{STUNT (Ours)}}& -           & \textbf{72.69} & \textbf{40.40} & \textbf{85.45} & \textbf{88.42} & \textbf{69.88} & \textbf{73.02} & \textbf{89.08} & \multicolumn{1}{c|}{{79.18}} & \textbf{74.77} \\ \bottomrule
\end{tabular}
}
\end{table}

